Matching the Clinical Reality: Accurate OCT-Based Diagnosis From Few Labels

Unlabeled data is often abundant in the clinic, making machine learning methods based on semi-supervised learning a good match for this setting. Despite this, they are currently receiving relatively little attention in medical image analysis literature. Instead, most practitioners and researchers focus on supervised or transfer learning approaches. The recently proposed MixMatch and FixMatch algorithms have demonstrated promising results in extracting useful representations while requiring very few labels. Motivated by these recent successes, we apply MixMatch and FixMatch in an ophthalmological diagnostic setting and investigate how they fare against standard transfer learning. We find that both algorithms outperform the transfer learning baseline on all fractions of labelled data. Furthermore, our experiments show that exponential moving average (EMA) of model parameters, which is a component of both algorithms, is not needed for our classification problem, as disabling it leaves the outcome unchanged. Our code is available online: https://github.com/Valentyn1997/oct-diagn-semi-supervised

==> slides/conclusion.tex <==
\section{Conclusion}
\begin{frame}{Conclusion}
    % Conclusion:
    \begin{itemize}
        \item we demonstrate the efficacy of
        \textbf{MixMatch} and \textbf{FixMatch}, when applied to an ophthalmological diagnostic problem on OCT data
        \item achieving over 80\% on as little as 40 labelled samples
        \item both algorithms outperform transfer learning in the few labelled data settings
    \end{itemize}
    
    % \vspace{1cm}
    % Future work:
    % \begin{itemize}
    %     \item try out few-shot deep learning
    % \end{itemize}

\end{frame}

==> slides/methodology.tex <==
\section{Methodology}

\subsection{Dataset}
\begin{frame}{Methodology: Dataset}
    \begin{columns}[onlytextwidth]
        \column{0.60\linewidth}
        For image classification task we use the \textbf{UCSD dataset} published by Kermany et al. \cite{kermany2018identifying}:
        \begin{itemize}
            \item 84K labelled optical coherence tomography (OCT) b-scans
            \item 4 classes: "normal”, “drusenoid” (DRUSEN), “choroidal neovascularization” (CNV) and “diabetic macular edema” (DME)
            \item median image size: 496$\times$512 pixels
        \end{itemize}
        
        \vspace{0.25cm}
        \column{0.35\linewidth}
        \begin{figure}
            \centering
            \includegraphics[width=\linewidth]{figures/dataset_sample.pdf}
            \vspace{-1cm}
            \caption{Sample from UCSD dataset}
        \end{figure}
    \end{columns}

\end{frame}

\subsection{Labelled / Unlabelled Images}
\begin{frame}{Methodology: Labelled / Unlabelled Images}
    Train/validation/test splits are taken from \href{https://www.kaggle.com/paultimothymooney/kermany2018}{Kaggle}. We vary the number of \textbf{labelled data}, which we sample randomly and in a balanced way from the training subset
    
    \hspace{0.25cm}
    \begin{figure}
        \centering
        \includegraphics[width=0.96\linewidth]{figures/dataset_dist.pdf}
        \vspace{-0.5cm}
        \caption{\scriptsize Count plots for dataset split. Dashed line shows labelled-unlabelled data split: upper part = unlabelled subset}
    \end{figure}

\end{frame}


\subsection{Realistic Evaluation}
\begin{frame}{Methodology: Realistic Evaluation}
    Our work follows the principles of the fair SSL evaluation framework, defined by Oliver et al. \cite{oliver2018realistic}:
    \begin{itemize}
        \item the same classifying backbone across all experiments: \\ \textbf{Wide ResNet-50-2} \cite{DBLP:journals/corr/ZagoruykoK16}
        \item SSL methods are compared with well-fine-tuned transfer learning / fully-supervised models
        \item unlabelled data from the same distribution
        \item realistically small validation subset (32 images)
    \end{itemize}

\end{frame}

==> slides/models.tex <==
\section{Experiments}

\subsection{Transfer Learning}
\begin{frame}{Experiments: Transfer Learning}
    \begin{columns}[onlytextwidth]
            \column{0.40\linewidth}
            We use an ImageNet pre-trained network with 2 settings:
            \vspace{0.5cm}
            \begin{itemize}
                \item<1-> \textbf{Feature extraction}. Freezing all parameters except the last FC layer
                \item<2-> \textbf{Fine-tuning}. Using the pre-trained network as the initialization, all parameters are trainable
            \end{itemize}
            
            \column{0.57\linewidth}
            
            \only<1>{\begin{figure}
                \vspace{-1cm}
                \centering
                
                \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
                
                \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
                %uncomment if require: \path (0,675); %set diagram left start at 0, and has height of 675
                
                %Shape: Rectangle [id:dp02499501479297561] 
                \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (200,120) -- (280,120) -- (280,152) -- (200,152) -- cycle ;
                %Shape: Rectangle [id:dp6032711133435942] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (320.5,120) -- (464,120) -- (464,152) -- (320.5,152) -- cycle ;
                %Straight Lines [id:da23699555871527145] 
                \draw    (290,134.5) -- (304,134.5)(290,137.5) -- (304,137.5) ;
                \draw [shift={(312,136)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Shape: Rectangle [id:dp3952040464476121] 
                \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (200,208) -- (280,208) -- (280,240) -- (200,240) -- cycle ;
                %Straight Lines [id:da3427801915013837] 
                \draw    (290,222.5) -- (304,222.5)(290,225.5) -- (304,225.5) ;
                \draw [shift={(312,224)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Shape: Rectangle [id:dp5566313884207257] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (320,208) -- (440,208) -- (440,240) -- (320,240) -- cycle ;
                %Straight Lines [id:da7636743259204934] 
                \draw    (320,160) -- (440,160) ;
                \draw [shift={(440,160)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
                \draw [shift={(320,160)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
                %Shape: Rectangle [id:dp046721072267932984] 
                \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (440,208) -- (464,208) -- (464,240) -- (440,240) -- cycle ;
                %Straight Lines [id:da8756747802120037] 
                \draw    (387,184) -- (387,198) ;
                \draw [shift={(387,200)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da002889173388934685] 
                \draw  [dash pattern={on 4.5pt off 4.5pt}]  (451,160) -- (451,198) ;
                \draw [shift={(451,200)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Shape: Rectangle [id:dp7072734523583166] 
                \draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ] (200,272) -- (464,272) -- (464,328) -- (200,328) -- cycle ;
                
                % Text Node
                \draw (212,94) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Dataset};
                % Text Node
                \draw (327,95) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Classifying backbone};
                % Text Node
                \draw (370,247) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Fixed};
                % Text Node
                \draw (379,128) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$ $$\displaystyle A$};
                % Text Node
                \draw (208,127) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {ImageNet};
                % Text Node
                \draw (219,215) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {UCSD};
                % Text Node
                \draw (378,162) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle A'$};
                % Text Node
                \draw (379,215) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle A'$};
                % Text Node
                \draw (427,247) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Trainable};
                % Text Node
                \draw (455,167) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Init};
                
                
                \end{tikzpicture}
            \end{figure}}

            \only<2>{\begin{figure}
                \vspace{-1cm}
                \centering

                \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
                
                \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
                %uncomment if require: \path (0,675); %set diagram left start at 0, and has height of 675
                
                %Shape: Rectangle [id:dp5521326104598689] 
                \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (200,408) -- (280,408) -- (280,440) -- (200,440) -- cycle ;
                %Shape: Rectangle [id:dp8195516485160681] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (320.5,408) -- (464,408) -- (464,440) -- (320.5,440) -- cycle ;
                %Straight Lines [id:da5530938883331571] 
                \draw    (290,422.5) -- (304,422.5)(290,425.5) -- (304,425.5) ;
                \draw [shift={(312,424)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Shape: Rectangle [id:dp8527259258948847] 
                \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.31 ][fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.28 ] (200,496) -- (280,496) -- (280,528) -- (200,528) -- cycle ;
                %Straight Lines [id:da021418490738524643] 
                \draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.31 ][fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.28 ]   (290,510.5) -- (304,510.5)(290,513.5) -- (304,513.5) ;
                \draw [shift={(312,512)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.31 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Shape: Rectangle [id:dp43320938284376576] 
                \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.31 ][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.28 ] (320,496) -- (440,496) -- (440,528) -- (320,528) -- cycle ;
                %Shape: Rectangle [id:dp4346794690496252] 
                \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.31 ][fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.28 ] (440,496) -- (464,496) -- (464,528) -- (440,528) -- cycle ;
                %Shape: Rectangle [id:dp2916290132278425] 
                \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (200,560) -- (280,560) -- (280,592) -- (200,592) -- cycle ;
                %Straight Lines [id:da3076153214946682] 
                \draw    (288.5,574.5) -- (304,574.5)(288.5,577.5) -- (304,577.5) ;
                \draw [shift={(312,576)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Shape: Rectangle [id:dp868079167873929] 
                \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (320.5,560) -- (464,560) -- (464,592) -- (320.5,592) -- cycle ;
                %Straight Lines [id:da10994440905158176] 
                \draw  [dash pattern={on 4.5pt off 4.5pt}]  (392,448) -- (392,550) ;
                \draw [shift={(392,552)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                
                % Text Node
                \draw (212,382) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Dataset};
                % Text Node
                \draw (327,383) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Classifying backbone};
                % Text Node
                \draw (370,535) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.1 ] [align=left] {Fixed};
                % Text Node
                \draw (379,416) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$ $$\displaystyle A$};
                % Text Node
                \draw (208,415) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {ImageNet};
                % Text Node
                \draw (219,503) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.1 ] [align=left] {UCSD};
                % Text Node
                \draw (379,503) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.1 ] [align=left] {$\displaystyle A'$};
                % Text Node
                \draw (427,535) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.1 ] [align=left] {Trainable};
                % Text Node
                \draw (367,597) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Trainable};
                % Text Node
                \draw (399,487) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Init};
                % Text Node
                \draw (219,567) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {UCSD};
                
                
                \end{tikzpicture}

            \end{figure}}
            
    \end{columns}
\end{frame}

\subsection{Semi-supervised Learning}
\begin{frame}{Experiments: Semi-supervised Learning}
    \begin{columns}[onlytextwidth]
            \column{0.4\linewidth}
            \textbf{MixMatch} \cite{berthelot2019mixmatch} (2019) -- teacher-student architecture:
            \begin{itemize}
                \item weak augmentations (flip-and-shift) $->$ consistency regularization
                \item soft pseudo-labeling of unlabelled augmented data with sharpening
                \item images and targets Mix-Ups $->$ linear behavior between training samples
                \item optional improvements: parameters EMA, linear rump-up for $\lambda_U$
            \end{itemize}
            
            \column{0.57\linewidth}
            \begin{figure}
                \centering
                \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
                
                \begin{tikzpicture}[scale=0.72,every node/.style={scale=0.72},x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
                %uncomment if require: \path (0,1509); %set diagram left start at 0, and has height of 1509
                
                %Image [id:dp0030498190467111996] 
                \draw (174.34,829.45) node  {\includegraphics[width=33.52pt,height=34.36pt]{figures/DRUSEN-9894035-18.jpeg}};
                %Image [id:dp8068131283301074] 
                \draw (53.93,828.36) node  {\includegraphics[width=32.9pt,height=29.45pt]{figures/DRUSEN-9894035-40.jpeg}};
                %Image [id:dp8667674934720351] 
                \draw (116.97,730.18) node  {\includegraphics[width=34.76pt,height=39.27pt]{figures/CNV-81630-7.jpeg}};
                %Image [id:dp626932977963329] 
                \draw (124.41,740) node  {\includegraphics[width=33.52pt,height=34.36pt]{figures/CNV-13823-5.jpeg}};
                %Image [id:dp04129319965587186] 
                \draw (131.45,743.27) node  {\includegraphics[width=32.9pt,height=29.45pt]{figures/NORMAL-12494-10.jpeg}};
                
                %Straight Lines [id:da4401570635200758] 
                \draw    (120,784) -- (97.2,814.4) ;
                \draw [shift={(96,816)}, rotate = 306.87] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da9257368714251086] 
                \draw    (120,784) -- (142.8,814.4) ;
                \draw [shift={(144,816)}, rotate = 233.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Image [id:dp4571105014094554] 
                \draw (63.17,839.27) node  {\includegraphics[width=34.76pt,height=39.27pt]{figures/NORMAL-12494-12.jpeg}};
                %Image [id:dp6703293695085264] 
                \draw (73.66,849.09) node  {\includegraphics[width=33.52pt,height=34.36pt]{figures/NORMAL-12494-20.jpeg}};
                %Image [id:dp8286486927185766] 
                \draw (181.93,834.91) node  {\includegraphics[width=32.9pt,height=29.45pt]{figures/NORMAL-15307-6.jpeg}};
                %Image [id:dp25360648353110826] 
                \draw (191.17,845.82) node  {\includegraphics[width=34.76pt,height=39.27pt]{figures/NORMAL-24500-5.jpeg}};
                %Straight Lines [id:da24523224073171734] 
                \draw    (64,880) -- (64,894) ;
                \draw [shift={(64,896)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da21077575285272876] 
                \draw    (192,880) -- (192,894) ;
                \draw [shift={(192,896)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Shape: Rectangle [id:dp3968074409259139] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (48,909.33) -- (56,909.33) -- (56,936) -- (48,936) -- cycle ;
                %Shape: Rectangle [id:dp2988277872758103] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (56,920) -- (64,920) -- (64,936) -- (56,936) -- cycle ;
                %Shape: Rectangle [id:dp8463780811416188] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (64,914.67) -- (72,914.67) -- (72,936) -- (64,936) -- cycle ;
                %Shape: Rectangle [id:dp5068725445633913] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (72,904) -- (80,904) -- (80,936) -- (72,936) -- cycle ;
                
                %Shape: Rectangle [id:dp8759467753112862] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (176,909.33) -- (184,909.33) -- (184,936) -- (176,936) -- cycle ;
                %Shape: Rectangle [id:dp10840697001287491] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (184,904) -- (192,904) -- (192,936) -- (184,936) -- cycle ;
                %Shape: Rectangle [id:dp6327374400678576] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (192,914.67) -- (200,914.67) -- (200,936) -- (192,936) -- cycle ;
                %Shape: Rectangle [id:dp9268403460713304] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (200,928) -- (208,928) -- (208,936) -- (200,936) -- cycle ;
                
                %Straight Lines [id:da02087547850310756] 
                \draw    (64,944) -- (102.14,959.26) ;
                \draw [shift={(104,960)}, rotate = 201.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da9285205725041903] 
                \draw    (192,944) -- (145.9,959.37) ;
                \draw [shift={(144,960)}, rotate = 341.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Shape: Rectangle [id:dp10535669840709772] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (104,984) -- (112,984) -- (112,992) -- (104,992) -- cycle ;
                %Shape: Rectangle [id:dp11734043843972919] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (112,960) -- (120,960) -- (120,992) -- (112,992) -- cycle ;
                %Shape: Rectangle [id:dp8346975824607779] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (120,976) -- (128,976) -- (128,992) -- (120,992) -- cycle ;
                %Shape: Rectangle [id:dp42299802970459344] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (128,984) -- (136,984) -- (136,992) -- (128,992) -- cycle ;
                
                %Image [id:dp44189897280793167] 
                \draw (355.59,730.18) node  {\includegraphics[width=34.76pt,height=39.27pt]{figures/DRUSEN-9894035-18.jpeg}};
                %Image [id:dp7079225647795759] 
                \draw (366.34,742.91) node  {\includegraphics[width=33.52pt,height=34.36pt]{figures/CNV-13823-5.jpeg}};
                %Image [id:dp7217455381715401] 
                \draw (377,753) node  {\includegraphics[width=34.5pt,height=34.5pt]{figures/Screenshot 2020-10-06 at 00.42.05.png}};
                %Straight Lines [id:da5533499664620138] 
                \draw    (320,784) -- (273.66,814.89) ;
                \draw [shift={(272,816)}, rotate = 326.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da6953868168747113] 
                \draw    (344,784) -- (390.34,814.89) ;
                \draw [shift={(392,816)}, rotate = 213.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da892774354693054] 
                \draw    (272,872) -- (310.29,894.97) ;
                \draw [shift={(312,896)}, rotate = 210.96] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da7290573359491499] 
                \draw    (392,872) -- (345.79,895.11) ;
                \draw [shift={(344,896)}, rotate = 333.43] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                
                % Text Node
                \draw (95,683) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\large Teacher}};
                % Text Node
                \draw (308,679) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\large Student};
                % Text Node
                \draw (23,719) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{43.551892pt}\setlength\topsep{0pt}
                \begin{center}
                Unlabelled \\data
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (83,763) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{57.1625pt}\setlength\topsep{0pt}
                \begin{center}
                Augmentations
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (87,878) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{53.528784pt}\setlength\topsep{0pt}
                \begin{center}
                Soft \\pseudo-labels
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (159,955) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{51.499392pt}\setlength\topsep{0pt}
                \begin{center}
                Averaging \\+ Sharpening
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (260,711) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{50.751892000000005pt}\setlength\topsep{0pt}
                \begin{center}
                Shuffled\\MixedUp\\ Augmented train data
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (239,823) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{49.661216pt}\setlength\topsep{0pt}
                \begin{center}
                $\displaystyle L_{U} \ =\ MSE$
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (331,823) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{89.90892000000001pt}\setlength\topsep{0pt}
                \begin{center}
                $\displaystyle L_{L} \ =\ Cross-Entropy$
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (231,845) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{58.06560800000001pt}\setlength\topsep{0pt}
                \begin{center}
                Unlabelled loss
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (363,841) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{50.362500000000004pt}\setlength\topsep{0pt}
                \begin{center}
                Labelled loss
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (294,902) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{64.419392pt}\setlength\topsep{0pt}
                \begin{center}
                $\displaystyle L\ =\ L_{l} +\lambda _{U} L_{U}$
                \end{center}
                
                \end{minipage}};
                
                
                \end{tikzpicture}

            \end{figure}
    \end{columns}
\end{frame}

\begin{frame}{Experiments: Semi-supervised Learning}
    \begin{columns}[onlytextwidth]
            \column{0.37\linewidth}
            \textbf{FixMatch} \cite{Sohn2020FixMatchSS} (2020) -- teacher-student architecture:
            \begin{itemize}
                \item weak augmentations (flip-and-shift) and strong augmentations (e.g. affine trasformations, color-jittering)
                \item hard pseudo-labeling of unlabelled weakly-augmented data
                \item threshold considers only confident pseudo-labels
                \item parameters EMA
            \end{itemize}
            
            \column{0.6\linewidth}
            \begin{figure}
                \centering
                \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
                
                \begin{tikzpicture}[scale=0.71,every node/.style={scale=0.71},x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
                %uncomment if require: \path (0,1509); %set diagram left start at 0, and has height of 1509
                
                
                %Image [id:dp38299383415644583] 
                \draw (302.34,1262.91) node  {\includegraphics[width=33.52pt,height=34.36pt]{figures/Screenshot 2020-10-06 at 00.42.05.png}};
                %Image [id:dp6985824233936637] 
                \draw (312.5,1272.5) node  {\includegraphics[width=35.25pt,height=35.25pt]{figures/NORMAL-2444883-34.jpeg}};
                %Image [id:dp3593502692595447] 
                \draw (325,1280) node  {\includegraphics[width=40.5pt,height=36pt]{figures/NORMAL-2448954-7.jpeg}};
                
                %Image [id:dp05432340088793941] 
                \draw (117.93,1252.36) node  {\includegraphics[width=32.9pt,height=29.45pt]{figures/DRUSEN-9894035-18.jpeg}};
                %Image [id:dp7218028793364208] 
                \draw (127.17,1263.27) node  {\includegraphics[width=34.76pt,height=39.27pt]{figures/CNV-13823-5.jpeg}};
                %Image [id:dp9817000992786233] 
                \draw (137.66,1273.09) node  {\includegraphics[width=33.52pt,height=34.36pt]{figures/NORMAL-15307-6.jpeg}};
                
                %Image [id:dp3623136626833261] 
                \draw (228.97,1143.27) node  {\includegraphics[width=34.76pt,height=39.27pt]{figures/NORMAL-12494-10.jpeg}};
                %Image [id:dp026111019718063844] 
                \draw (236.41,1153.09) node  {\includegraphics[width=33.52pt,height=34.36pt]{figures/NORMAL-12494-12.jpeg}};
                %Image [id:dp2868912309026661] 
                \draw (243.45,1156.36) node  {\includegraphics[width=32.9pt,height=29.45pt]{figures/CNV-81630-7.jpeg}};
                
                %Straight Lines [id:da8672235691282764] 
                \draw    (216,1184) -- (169.41,1230.59) ;
                \draw [shift={(168,1232)}, rotate = 315] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da7667547851918368] 
                \draw    (240,1184) -- (278.72,1230.46) ;
                \draw [shift={(280,1232)}, rotate = 230.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da4810462651058949] 
                \draw    (128,1304) -- (128,1318) ;
                \draw [shift={(128,1320)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da036142325850258006] 
                \draw    (128,1360) -- (128,1374) ;
                \draw [shift={(128,1376)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Shape: Rectangle [id:dp3565290102846346] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (112,1328) -- (120,1328) -- (120,1352) -- (112,1352) -- cycle ;
                %Shape: Rectangle [id:dp04856899469706266] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (120,1336) -- (128,1336) -- (128,1352) -- (120,1352) -- cycle ;
                %Shape: Rectangle [id:dp04300562858447843] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (128,1330.67) -- (136,1330.67) -- (136,1352) -- (128,1352) -- cycle ;
                %Shape: Rectangle [id:dp7129343384580189] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (136,1312) -- (144,1312) -- (144,1352) -- (136,1352) -- cycle ;
                
                %Image [id:dp9287650042681281] 
                \draw (439.17,1138.18) node  {\includegraphics[width=34.76pt,height=39.27pt]{figures/DRUSEN-9894035-18.jpeg}};
                %Image [id:dp8911240067680881] 
                \draw (449.93,1150.91) node  {\includegraphics[width=33.52pt,height=34.36pt]{figures/DRUSEN-9894035-40.jpeg}};
                %Image [id:dp5516520165150292] 
                \draw (460.59,1161) node  {\includegraphics[width=34.5pt,height=34.5pt]{figures/NORMAL-12494-20.jpeg}};
                %Straight Lines [id:da8436138252631613] 
                \draw    (480,1192) -- (480,1302) ;
                \draw [shift={(480,1304)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da5973098860487132] 
                \draw    (320,1352) -- (358.44,1382.75) ;
                \draw [shift={(360,1384)}, rotate = 218.66] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Straight Lines [id:da15077464726223044] 
                \draw    (472,1352) -- (433.56,1382.75) ;
                \draw [shift={(432,1384)}, rotate = 321.34000000000003] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
                %Shape: Rectangle [id:dp2440978292792535] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.18 ] (112,1400) -- (120,1400) -- (120,1424) -- (112,1424) -- cycle ;
                %Shape: Rectangle [id:dp30002506631986847] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.25 ] (120,1408) -- (128,1408) -- (128,1424) -- (120,1424) -- cycle ;
                %Shape: Rectangle [id:dp612853876461541] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.2 ] (128,1402.67) -- (136,1402.67) -- (136,1424) -- (128,1424) -- cycle ;
                %Shape: Rectangle [id:dp39103373336398173] 
                \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (136,1384) -- (144,1384) -- (144,1424) -- (136,1424) -- cycle ;
                %Straight Lines [id:da5540390825212667] 
                \draw  [dash pattern={on 4.5pt off 4.5pt}]  (104,1392) -- (152,1392) ;
                
                % Text Node
                \draw (151,1091) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\large Teacher}};
                % Text Node
                \draw (367,1090) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {Student};
                % Text Node
                \draw (135,1132.09) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{43.551892pt}\setlength\topsep{0pt}
                \begin{center}
                Unlabelled \\data
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (108,1183) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{47.228108000000006pt}\setlength\topsep{0pt}
                \begin{center}
                {\small Weak }\\{\small augmentation}
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (151,1311) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{53.528784pt}\setlength\topsep{0pt}
                \begin{center}
                Soft\\pseudo-labels
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (135,1359) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{49.895pt}\setlength\topsep{0pt}
                \begin{center}
                Thresholding
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (489.59,1127) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{33.575pt}\setlength\topsep{0pt}
                \begin{center}
                Labelled\\Data
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (411,1311) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{89.90892000000001pt}\setlength\topsep{0pt}
                \begin{center}
                $\displaystyle L_{L} \ =\ Cross-Entropy$
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (443,1329) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{50.362500000000004pt}\setlength\topsep{0pt}
                \begin{center}
                Labelled loss
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (344,1391) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{64.419392pt}\setlength\topsep{0pt}
                \begin{center}
                $\displaystyle L\ =\ L_{l} +\lambda _{U} L_{U}$
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (271,1183) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{47.228108000000006pt}\setlength\topsep{0pt}
                \begin{center}
                {\small Strong }\\{\small augmentation}
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (152,1383) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{53.528784pt}\setlength\topsep{0pt}
                \begin{center}
                Hard\\pseudo-labels
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (394,1215) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{47.228108000000006pt}\setlength\topsep{0pt}
                \begin{center}
                {\small Weak }\\{\small augmentation}
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (279,1327) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{58.06560800000001pt}\setlength\topsep{0pt}
                \begin{center}
                Unlabelled loss
                \end{center}
                
                \end{minipage}};
                % Text Node
                \draw (255,1310) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{91.34304pt}\setlength\topsep{0pt}
                \begin{center}
                $\displaystyle L_{U} \ =\ Cross-Entropy$
                \end{center}
                
                \end{minipage}};
                
                
                \end{tikzpicture}


            \end{figure}
    \end{columns}

\end{frame}

\subsection{Comparison}
\begin{frame}{Experiments: Comparison}
    \begin{columns}[onlytextwidth]
        \column{0.47\linewidth}
        \begin{figure}
            \hspace{-0.9cm}
            \centering
            \includegraphics[width=1.1\linewidth]{figures/best_models.pdf}
            \caption{\scriptsize Best models, test performance after two-fold hyperparameter search}
            \label{fig:best_models}
        \end{figure}
        
        \column{0.51\linewidth}
        
        \begin{table}
            \hspace{-0.75cm}
            \centering
            \scriptsize
            \setlength{\tabcolsep}{2pt}
            \renewcommand{\arraystretch}{1}
            \begin{tabular}{l|l|l|l}
                 \toprule
                 Method & $n_l$ & Accuracy & Notes \\ \midrule
                 Kermany et al. \cite{kermany2018identifying} & All & 96.6\% & Original paper \\ \hline
                 Alqudah \cite{alqudah2020aoct}
                 & All & 97.1\% & \pbox{15cm}{\vspace{4pt} Extended UCSD \\ with 5 classes \vspace{4pt}}  \\ \hline
                 Wu et al. \cite{wu2020attennet} & All & 97.5\% \\ \hline
                 Chetoui et al. \cite{chetoui2020deep} & All & 98.46\% \\ \hline
                 Tsuji et al.\cite{tsuji2020classification} & All & 99.6\% \\ \hline
                 \pbox{10cm}{\vspace{4pt}\textbf{WideResNet-50-2} \\ \textbf{(with EMA)}} & All & \textbf{99.69\%} & \pbox{15cm}{\vspace{4pt} With EMA decay \\ (${\beta_{\text{EMA}}} = 0.999$) \vspace{4pt}}   \\ \midrule
        %         & 100 & 86.29 $\pm$ 1.83\%\\ 
        %         Das et al. \cite{das2020data} & 300 & 95.31 $\pm$ 1.18 \%\\
        %          & 500 & 97.43 $\pm$ 0.66\%\\ \hline
                  He et al. \cite{he2020retinal} & 835 & 87.25\% * & *Average precision \\
                 \bottomrule
            \end{tabular}
            % \vspace{0.15cm}
            \caption{Reported test accuracies for UCSD dataset}
            \label{table:reported-results}
        \end{table}
    \end{columns}
\end{frame}

\subsection{Additional Findings}
\begin{frame}{Experiments: Additional Findings}
    \begin{columns}[onlytextwidth]
        \column{0.48\linewidth}
        \textbf{Parameters Exponential Moving Average (EMA)} is an inherent part of Fix-Match and an optional for MixMatch:
        \begin{itemize}
            \item we observe learning curves to be more stable for both train and validation subsets
            \item validation subset is well-chosen $->$ variability could be advantageous
            \item on UCSD -- no obvious advantage of its usage 
        \end{itemize}
        
        
        \column{0.48    \linewidth}
        \textbf{Transfer learning approaches}:
        \begin{itemize}
            \item fine-tuning outperforms feature extraction approach in all label settings
            \item original models are trained on the dataset with RGB channels $->$ better adaptability to monochrome images in full network fine-tuning
        \end{itemize}
        
    \end{columns}
\end{frame}

==> slides/motivation.tex <==
\section{Motivation}

\subsection{Few Labels Problem}
\begin{frame}{Motivation: Few Labels Problem}
\begin{columns}[onlytextwidth]
    \column{0.65\linewidth}
    
    \textbf{Supervised learning} is difficult to apply in the medical domain:
    \begin{itemize}
        % \setlength\itemsep{1em}
        \item high cost of data labelling:
        \begin{itemize}
            \item requires experts with domain knowledge
            \item more fine-grained problem formulations (e.g. volume level vs. slice level) $->$ exponential growth of cost
        \end{itemize}
        
        \item epistemic uncertainty: data with high  inter-annotator agreement is required \cite{lampert2016empirical}
    \end{itemize}
    
    \vspace{0.25cm}

    \column{0.25\linewidth}
    \begin{figure}
        \centering
        \includegraphics[width=\linewidth]{figures/journal.pone.0220063.g003.PNG}
        \vspace{-0.5cm}
        \caption{\href{https://journals.plos.org/plosone/article?id=10.1371/journal.pone.0220063}{\tiny Automated OCT image compartmentalization}}
    \end{figure}
\end{columns}
\end{frame}

\subsection{Usage of Unlabelled Data}
\begin{frame}{Motivation: Usage of Unlabelled Data}
    \textbf{Transfer Learning} is often used in few labels setting:
    \begin{itemize}
        \item the possibility of knowledge transfer to medical data is questionable
        \item ignorance of (abundant) \textbf{unlabeled data}
    \end{itemize}
    
    \vspace{0.25cm}
    SOTA \textbf{Semi-supervised learning} (SSL) algorithms show a promising results on the benchmark datasets $->$ Incentives to employ SSL

\end{frame}
